Shared Control with Black Box Agents using Oracle Queries

Shared control problems involve a robot learning to collaborate with a human. When learning a shared control policy, short communication between the agents can often significantly reduce running times and improve the system's accuracy. We extend the shared control problem to include the ability to directly query a cooperating agent. We consider two types of potential responses to a query, namely oracles: one that can provide the learner with the best action they should take, even when that action might be myopically wrong, and one with a bounded knowledge limited to its part of the system. Given this additional information channel, this work further presents three heuristics for choosing when to query: reinforcement learning-based, utility-based, and entropy-based. These heuristics aim to reduce a system's overall learning cost. Empirical results on two environments show the benefits of querying to learn a better control policy and the tradeoffs between the proposed heuristics.

==> Figures/Automata/automaton_cases.tex <==

 
% required packages and libraries


\begin{tikzpicture}[node distance=15mm, auto]
  % first automaton
  \node[state,initial]   (c0)                 {$c_0$};
  \node[state]           (c1) [right of=c0]      {$c_1$};
  
  \path[-stealth] 
    (c0) edge[bend left] node {$a$}
    (c1)
    (c1) edge[bend left] node {$b$,$c$}  (c0);
   

 \end{tikzpicture}

 \begin{tikzpicture}[node distance=15mm, auto]
 
  % second automaton

   
    
    
    \node[state, initial](e0)  {$ e_0$};
    \node[state, below right of=e0] (e2) {$e_2$};
    \node[state, below left of=e0] (e1) {$e_1$};
    \node[state, below of=e1]  (e3){$e_3$};
    \node[state, below of=e2] (e4) {$e_4$};
    
      \path[->] (e0) edge [left]node {$b$} (e1)
                (e0) edge [ right]node {$c$} (e2)
                (e1) edge [bend left]node {$a$} (e3)
                (e2) edge[bend left] node {$c$} (e4)
                (e4) edge[bend left] node {$a$} (e2)
                (e3) edge[bend left] node {$b$} (e1);
                %(s2) edge node {$b$} (s4)
                %(s4) edge [loop below] node {$a$,$b$} (s4);
            
\end{tikzpicture}


==> Figures/Automata/automaton_combination.tex <==
 

 \begin{tikzpicture}[node distance=15mm, auto]
  % first automaton
  \node[state,initial]   (c0)               {$c_0$};
  \node[state]           (c1) [right of=c0]      {$c_1$};
  \node[state]           (c2) [right of=c1]      {$c_2$};
  \node[state]           (c3) [right of=c2]      {$c_3$};
  \path[-stealth] (c0) edge[bend left] node {$a$,$b$}(c1)
    (c1) edge[bend left] node {$a$,$b$}  (c2)
    (c2) edge[bend left] node {$a$,$b$}  (c3)
    (c3) edge [loop above]  node {c}();

  % second automaton
  \node[state,initial]   (e0) [below=15mm of c0] {$e_0$};
  \node[state]           (e1) [right of=e0]      {$e_1$};
  \node[state]           (e2) [right of=e1]      {$e_2$};
  \node[state]           (e3) [right of=e2]      {$e_3$};
 
  \node[state]           (e4) [below of=e1]      {$e_4$};
  \path[->] (e0) edge node {$a$} (e1)
            (e1) edge node {$b$} (e2)
            (e2) edge node {$a$} (e3)
            (e3) edge [loop above] node {$c$} (e3)
            (e0) edge node[left] {$b$} (e4)
            (e1) edge node {$a$} (e4)
            (e2) edge node[right] {$b$} (e4)
            (e4) edge [loop below] node {$a$,$b$} (e4);
            
\end{tikzpicture}


==> Figures/Automata/automaton_strategy.tex <==

 \begin{tikzpicture}[node distance=15mm, auto]
  % first automaton
  \node[state,initial]   (c0)               {$c_0$};
  \node[state]           (c1) [below of=c0]      {$c_1$};
  \node[state]           (c2) [below left of=c1]      {$c_2$};
  \node[state]           (c3) [below right of=c1]      {$c_3$};
  \path[-stealth] (c0) edge node {$a$}(c1)
    (c1) edge[left] node {$b$}  (c2)
    (c1) edge[right] node {$c$}  (c3)
    (c2) edge [loop below]  node {$b$}()
    (c3) edge [loop below]  node {$c$}();
\end{tikzpicture}
 \begin{tikzpicture}[node distance=15mm, auto]
  % second automaton
  \node[state,initial]   (e0)  {$e_0$};
  \node[state]           (e1) [below left of=e0]      {$e_1$};
  \node[state]           (e2) [below right of=e0]      {$e_2$};
  \node[state]           (e3) [below of=e1]      {$e_3$};
  \node[state]           (e4) [below of=e2]      {$e_4$};
  \node[state]           (e5) [below of=e3]      {$e_5$};
  \node[state]           (e6) [below of=e4]      {$e_6$};
  \path[->] (e0) edge node[left] {$b$} (e1)
            (e0) edge node[right] {$c$} (e2)
            (e1) edge node {$a$} (e3)
            (e2) edge node {$a$} (e4)
            (e3) edge node {$c$} (e5)
            (e4) edge node {$b$} (e6)
            (e5) edge [loop below] node{$b$} (e5)
            (e6) edge [loop below] node {$c$} (e6);
            
\end{tikzpicture}

==> queryFig.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/IG cases use oracle.png}
         \caption{Entropy Heuristic on Cases.}
         \label{fig:IG_cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/IG strategy use oracle.png}
         \caption{Entropy Heuristic on Strategy.}
         \label{fig:IG_strategy}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/IG combination lock use oracle.png}
         \caption{Entropy Heuristic on Combination Lock.}
         \label{fig:IG_combination}
     \end{subfigure}


          \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/max prob cses use oracle.png}
         \caption{Utility Heuristic on Cases.}
         \label{fig:Util_cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/max prob strategy use oracle.png}
         \caption{Utility Heuristic on Strategy.}
         \label{fig:Util_strategy}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/max prob combination lock use oracle.png}
         \caption{Utility Heuristic on Combination Lock.}
         \label{fig:Util_combination}
     \end{subfigure}



          \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/Qlearning cases use oracle.png}
         \caption{RL Heuristic on Cases.}
         \label{fig:RL_cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/Qlearning s trategy use oracle.png}
         \caption{RL Heuristic on Strategy.}
         \label{fig:RL_strategy}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Queries/Qlearning combination lock use oracle.png}
         \caption{RL Heuristic on Combination Lock.}
         \label{fig:RL_combination}
     \end{subfigure}
        \caption{Number of Queries used per training episode. The results are cut after 15 episodes, as the algorithm converges.}
        \label{fig:IG_queries}
        \vspace{-4mm}
\end{figure*}
